Executable Behaviour and the \pi-Calculus (extended abstract)

Reactive Turing machines extend classical Turing machines with a facility to model observable interactive behaviour. We call a behaviour executable if, and only if, it is behaviourally equivalent to the behaviour of a reactive Turing machine. In this paper, we study the relationship between executable behaviour and behaviour that can be specified in the pi-calculus. We establish that all executable behaviour can be specified in the pi-calculus up to divergence-preserving branching bisimilarity. The converse, however, is not true due to (intended) limitations of the model of reactive Turing machines. That is, the pi-calculus allows the specification of behaviour that is not executable up to divergence-preserving branching bisimilarity. Motivated by an intuitive understanding of executability, we then consider a restriction on the operational semantics of the pi-calculus that does associate with every pi-term executable behaviour, at least up to the version of branching bisimilarity that does not require the preservation of divergence.

==> eptcsdata.tex <==
\providecommand{\firstpage}{37}
\providecommand{\publicationstatus}{S. Knight, I. Lanese, A. Lluch Lafuente and H. T. Vieira (Eds.):\\ 8th Interaction and Concurrency Experience (ICE 2015)\\
EPTCS 189, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.189.5}{10.4204/EPTCS.189.5}}

